Explaining by Imitating: Understanding Decisions by Interpretable Policy Learning

Understanding human behavior from observed data is critical for transparency and accountability in decision-making. Consider real-world settings such as healthcare, in which modeling a decision-maker's policy is challenging -- with no access to underlying states, no knowledge of environment dynamics, and no allowance for live experimentation. We desire learning a data-driven representation of decision-making behavior that (1) inheres transparency by design, (2) accommodates partial observability, and (3) operates completely offline. To satisfy these key criteria, we propose a novel model-based Bayesian method for interpretable policy learning ("Interpole") that jointly estimates an agent's (possibly biased) belief-update process together with their (possibly suboptimal) belief-action mapping. Through experiments on both simulated and real-world data for the problem of Alzheimer's disease diagnosis, we illustrate the potential of our approach as an investigative device for auditing, quantifying, and understanding human decision-making behavior.

==> figures/bias.tex <==
\begin{wraptable}{r}{.48\linewidth}
    \captionof{table}{\textit{Performance Comparison in BIAS.} \textsc{Interpole} is best. Belief mismatch is n/a to R-BC. $^\dagger$$\times 10^{-3}$}
    \label{tbl:bias}
    \smallskip\vspace{-\baselineskip}
    \resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{1.1}
        \begin{tabular}{@{}lS[table-format=2.1]@{$\,\pm\,$}S[table-format=1.2]S[table-format=3.1]@{$\,\pm\,$}S[table-format=2.1]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]@{}}
            \toprule
            \bf Algorithm & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Belief\\\bf Mismatch\smash{$^\dagger$}}}} & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Policy\\\bf Mismatch\smash{$^\dagger$}}}} & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Stopping\\\bf Time Error}}} \\
            \midrule
            R-BC & \multicolumn{2}{c}{--} & 191.8&78.8 & 2.22&0.45 \\
            PO-MB-IL & 83.2&3.03 & 125.4&18.4 & 3.80&0.19 \\
            PO-IRL & 83.2&3.03 & 144.0&29.4 & 3.46&0.22 \\
            Off.\,PO-IRL & 84.9&8.28 & 62.8&7.5 & 3.12&0.41 \\
            \midrule
            \textsc{Interpole} & 3.8&0.34 & 1.8&0.6 & 2.14&0.51 \\
            \bottomrule
        \end{tabular}}
\end{wraptable}


==> tables/adni.tex <==
\begin{wraptable}{r}{.48\linewidth}
    \centering
    \caption{\textit{Performance Comparison in ADNI.} \textsc{Interpole} is best/second-best for action-matching metrics.}
    \label{tbl:adni}
    \smallskip\vspace{-\baselineskip}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{@{}lS[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]@{}}
            \toprule
            \bf Algorithm & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Calibration\\\bf (Brier Score)}}} & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Area under\\\bf ROC Curve}}} & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Area under\\\bf PR Curve}}} \\
            \midrule
            R-BC & 0.18&0.05 & 0.61&0.05 & 0.81&0.08 \\
            PO-MB-IL & 0.19&0.07 & 0.54&0.07 & 0.79&0.11 \\
            PO-IRL & 0.23&0.01 & 0.51&0.07 & 0.78&0.09 \\
            Off.\,PO-IRL & 0.24&0.01 & 0.54&0.05 & 0.79&0.09 \\
            \midrule
            \textsc{Interpole} & 0.17&0.05 & 0.60&0.04 & 0.81&0.09 \\
            \bottomrule
        \end{tabular}}
\end{wraptable}

==> tables/bias.tex <==
\begin{wraptable}{r}{.48\linewidth}
    \centering
    \caption{\textit{Performance Comparison in BIAS.} \textsc{Interpole} is best. Belief mismatch is n/a to R-BC. $^\dagger$$\times 10^{-3}$}
    \label{tbl:bias}
    \smallskip\vspace{-\baselineskip}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lS[table-format=2.1]@{$\,\pm\,$}S[table-format=1.2]S[table-format=3.1]@{$\,\pm\,$}S[table-format=2.1]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]@{}}
        \toprule
        \bf Algorithm & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Belief\\\bf Mismatch\smash{$^\dagger$}}}} & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Policy\\\bf Mismatch\smash{$^\dagger$}}}} & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Stopping\\\bf Time Error}}} \\
        \midrule
        R-BC & \multicolumn{2}{c}{--} & 191.8&78.8 & 2.22&0.45 \\
        PO-MB-IL & 83.2&3.03 & 125.4&18.4 & 3.80&0.19 \\
        PO-IRL & 83.2&3.03 & 144.0&29.4 & 3.46&0.22 \\
        Off.\,PO-IRL & 84.9&8.28 & 62.8&7.5 & 3.12&0.41 \\
        \midrule
        \textsc{Interpole} & 3.8&0.34 & 1.8&0.6 & 2.14&0.51 \\
        \bottomrule
    \end{tabular}}
\end{wraptable}


==> tables/comparison.tex <==
\begin{table}
    \centering
    \caption{\textit{Performance Comparisons.} In ADNI, \textsc{Interpole} is first- or second-best for all action-matching metrics. In DIAG and BIAS, \textsc{Interpole} is best. 
    Belief/policy mismatch is not applicable to ADNI without ground-truth beliefs/policies. Belief mismatch is not applicable to R-BC. $^\dagger$$\times 10^{-3}$}
    \label{tbl:comparison}
    \tiny
    \vspace{-\baselineskip}
    \setlength{\tabcolsep}{2.4pt}
    \begin{tabularx}{\linewidth}{@{}XS[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]|S[table-format=2.1]@{$\,\pm\,$}S[table-format=2.1]S[table-format=2.1]@{$\,\pm\,$}S[table-format=2.1]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]|S[table-format=2.1]@{$\,\pm\,$}S[table-format=1.2]S[table-format=3.1]@{$\,\pm\,$}S[table-format=2.1]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]@{}}
        \toprule
        & \multicolumn{6}{c}{\bf ADNI} & \multicolumn{6}{c}{\bf DIAG} & \multicolumn{6}{c}{\bf BIAS} \\
        \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19}
        \bf Algorithm & \multicolumn{2}{c}{\makecell{\bf Calibration\\\bf (Brier Score)}} & \multicolumn{2}{c}{\makecell{\bf Area under\\\bf ROC Curve}} & \multicolumn{2}{c}{\makecell{\bf Area under\\\bf PR Curve}} & \multicolumn{2}{c}{\makecell{\bf Belief\\\bf Mismatch\smash{$^\dagger$}}} & \multicolumn{2}{c}{\makecell{\bf Policy\\\bf Mismatch\smash{$^\dagger$}}} & \multicolumn{2}{c}{\makecell{\bf Stopping\\\bf Time Error}} & \multicolumn{2}{c}{\makecell{\bf Belief\\\bf Mismatch\smash{$^\dagger$}}} & \multicolumn{2}{c}{\makecell{\bf Policy\\\bf Mismatch\smash{$^\dagger$}}} & \multicolumn{2}{c@{}}{\makecell{\bf Stopping\\\bf Time Error}} \\
        \midrule
        R-BC & 0.18&0.05 & 0.61&0.05 & 0.81&0.08 & \multicolumn{2}{c}{--} & 6.7&1.4 & 5.91&1.29 & \multicolumn{2}{c}{--} & 191.8&78.8 & 2.22&0.45 \\
        PO-MB-IL & 0.19&0.07 & 0.54&0.07 & 0.79&0.11 & 42.7&34.0 & 47.9&18.9 & 6.34&1.48 & 83.2&3.03 & 125.4&18.4 & 3.80&0.19 \\
        PO-IRL & 0.23&0.01 & 0.51&0.07 & 0.78&0.09 & 42.7&34.0 & 62.1&29.1 & 6.41&1.80 & 83.2&3.03 & 144.0&29.4 & 3.46&0.22 \\
        Off.\,PO-IRL& 0.24&0.01 & 0.54&0.05 & 0.79&0.09 & 26.1&5.6 & 2.1&0.2 & 5.42&0.69 & 84.9&8.28 & 62.8&7.5 & 3.12&0.41 \\
        \midrule
        \textsc{Interpole} & 0.17&0.05 & 0.60&0.04 & 0.81&0.09 & 0.6&0.1 & 0.8&0.2 & 5.38&1.14 & 3.8&0.34 & 1.8&0.6 & 2.14&0.51 \\
        \bottomrule
    \end{tabularx}
    \vspace{-1.5\baselineskip}
\end{table}


==> tables/diag.tex <==
\begin{wraptable}{r}{.48\linewidth}
    \centering
    \caption{\textit{Performance Comparison in DIAG.} \textsc{Interpole} is best. Belief mismatch is n/a to R-BC. $^\dagger$$\times 10^{-3}$}
    \label{tbl:diag}
    \smallskip\vspace{-\baselineskip}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lS[table-format=2.1]@{$\,\pm\,$}S[table-format=2.1]S[table-format=2.1]@{$\,\pm\,$}S[table-format=2.1]S[table-format=1.2]@{$\,\pm\,$}S[table-format=1.2]@{}}
        \toprule
        \bf Algorithm & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Belief\\\bf Mismatch\smash{$^\dagger$}}}} & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Policy\\\bf Mismatch\smash{$^\dagger$}}}} & \multicolumn{2}{c}{\makebox[0pt]{\makecell{\bf Stopping\\\bf Time Error}}} \\
        \midrule
        R-BC & \multicolumn{2}{c}{--} & 6.7&1.4 & 5.91&1.29 \\
        PO-MB-IL & 42.7&34.0 & 47.9&18.9 & 6.34&1.48 \\
        PO-IRL & 42.7&34.0 & 62.1&29.1 & 6.41&1.80 \\
        Off.\,PO-IRL & 26.1&5.6 & 2.1&0.2 & 5.42&0.69 \\
        \midrule
        \textsc{Interpole} & 0.6&0.1 & 0.8&0.2 & 5.38&1.14 \\
        \bottomrule
    \end{tabular}}
\end{wraptable}

